Poster: Communication in Open-Source Projects--End of the E-mail Era?

Communication is essential in software engineering. Especially in distributed open-source teams, communication needs to be supported by channels including mailing lists, forums, issue trackers, and chat systems. Yet, we do not have a clear understanding of which communication channels stakeholders in open-source projects use. In this study, we fill the knowledge gap by investigating a statistically representative sample of 400 GitHub projects. We discover the used communication channels by regular expressions on project data. We show that (1) half of the GitHub projects use observable communication channels; (2) GitHub Issues, e-mail addresses, and the modern chat system Gitter are the most common channels; (3) mailing lists are only in place five and have a lower market share than all modern chat systems combined.

==> comparison.tex <==
%!TEX root = main.tex

\subsubsection{Comparison of mailing lists}

\begin{figure*}[t!]
	\center
	\includegraphics[width=\textwidth]{figs/ml_cats_vs_subcats.pdf}
	\caption{The categories and subcategories we used for mailing lists.}
	\label{fig:ml-cats-and-subcats}
\end{figure*}

In contrast to Guzzi, the distribution of channels in our case was totally different. \textit{Usage} and \textit{discarded} were on the first two places and only then the \textit{implementation} category followed. As we did not have a look at only development mailing lists like Guzzi but at many different lists this seems reasonable. This also explains why the \textit{technical infrastructure} category was not used that often. Instead, the social part was much higher in our mailing lists. Apparently there is a difference between pure development mailing lists and general purpose lists which can be seen here. 

Inside the single categories there are also some differences. In the \textit{usage} category, the amount of references to \textit{external projects} was much smaller compared to the amount of \textit{problems and bugs} or \textit{information seeking}. Maybe Guzzi's mailing list was special about users sharing their external projects and this cannot be generalized. 

Also in the \textit{discarded} category the order was different but not much. In our case there were more \textit{turtle} than \textit{auto generated} messages. This highly depends on the list if auto generated messages are included or not. 

In the \textit{implementation} category every code in our list was found equally. Compared to Guzzi we found more \textit{feature suggestions} and less discussion. Also this can be explained by using not only development lists, as developers might just add features and discussions are difficult for non-developers. 

Interestingly, in the \textit{social interaction} category we did not use the codes \textit{social norm} and \textit{new contributors} at all. Instead we added two new codes, namely \textit{advertising} and \textit{donations}. 

We also found some differences in the \textit{technical infrastructure} category. We did not used the codes \textit{bug tracking, mailing list} or \textit{language} at all. 
Also the order was different. We saw more references to the \textit{website} but much less to \textit{versioning}. Again, the specific devloper mailing list seems to have other  focus than mailing lists in general. 

Last, in the \textit{project status} category we used the code \textit{release} much more often than the \textit{planning} code whereas in Guzzi's paper the codes were used nearly equally often. Again, in more general lists it might be more interesting to hear about releases as the developers might already know about them. 

Finally, we can say that we found quite some differences to Guzzi et al. One reason could be that Guzzi et al. only looked at one mailing list whereas we examined several lists. The code distribution of one list is apparently not generalizable to other lists. Also the usage of a mailing list highly depends on its purpose, e.g. is it a list for developers only or more a list for everybody. We think that our results show more generally what is shared over the channel mailing list. 

\subsubsection{General comparison}

In a general comparison of Guzzi and all examined communication channels the picture is not that different. 

Again, the distribution was different, namely the same as for mailing lists only. Apparently channels other than mailing lists are more used to ask about how to do something and bug reporting and a little less to suggest features and discuss implementation details. As we included issue trackers and forums in our search, it seems reasonable that the share of bugs and questions is higher than in a pure mailing list. Also the use of more social channels like Gitter or Twitter can explain the increase of the \textit{social interaction} category. 

Regarding the \textit{usage} category, the \textit{problems and bugs} code was even more often used than in the mailing lists only and the \textit{external projects} code's share was still very small. This hardens our thought that sharing an external project is not that common in general. 

Also in the \textit{discarded} category the order was the same as for mailing lists but the codes were used more often (whioch makes sense when coding more projects). 

In the \textit{implementation} category the codes were not equally share any more. The\textit{feature suggestions} was the most common code which could be seen mostly in github issues or on Gitter. Additionally we could see many \textit{development task}s, especially in Github issues. Again we think that ``normal'' users like to suggest features over many channels whereas development tasks can be collected in issue trackers. Discussion is only a small part of it. 

For the \textit{social interaction} category we could find all the codes from Guzzi plus the ones we added. \textit{Coordination} is still highly done through several channels. Though, \textit{new contributors} was used only a few times which might lead to the conclusion that not that many developers use the channels. 

In the \textit{project status} category we added a code about \textit{progress} as there were some messages about it. There are still more messages about releases than about planning but the difference is not as big as when comparing only the mailing lists. 

Finally, in the \textit{technical infrastructure} category, we added codes about \textit{chat} and \textit{code hosting}. There were less messages about \textit{versioning} but more about \textit{issue tracking} and the \textit{website}. We did not see any references to other \textit{mailing list}s. 

Regarding the role of the channels compared to the role of the mailing list we can confirm that issue trackers like JIRA are still used. In contrast to Guzzi we cannot confirm that IRC was used that often, but other chats like Slack or Gitter are highly used. 

Guzzi et al. stated that ``instead of using the mailing list, [developers] prefer to coordinate through items in the issue tracking system''\cite{guzzi2013}. We also found quite many repositories that used Github issues or external issue trackers and can confirm that these channels are used to report bugs and handle development tasks. On the other hand, the \textit{social interaction} category including the \textit{coordination} code was not found in many Github or external issue trackers. 


We agree that ``Overall, our study provides evidence that the communication channels work in parallel and they remain disconnected between one another, and that the development mailing list does not play (anymore) the role of a hub'' \cite{guzzi2013}.

Mailing lists are still important but the are not the main communication channel any more. 


Overall, we think that it makes a big difference if only developers use a channel or if it is open for everybody. Developers mainly focus on developing tasks whereas users report bugs, request features and ask questions about releases and stuff. Guzzi et al. did a great job summarizing their mailing list, but as we can see their results do not apply to the average mailing list or other communication channels. 


==> discussion.tex <==
%!TEX root = main.tex
\section{Discussion}
\label{sec:discussion}

\subsection{Impressions}

Keeping in mind that our sample contains projects that have at least 10 contributors, 
the implications are that either half of the GitHub projects are using a very wide spectrum of rarely frequently used communication channels or that half of the GitHub projects are at risk of being poorly coordinated 
or with a solo maintainer accepting contributions without any communication. 

GitHub Issues are arguably the easier communication channel to add to a GitHub project.
They are free and can be activated when creating the project, or anytime, by checking a single flag.
We were surprised to see a strong contrast in our data.
First, we estimate the overall adoption of GitHub Issues to be $17.5\%$ GitHub projects, 
meaning that less than a fifth of the GitHub projects within our definition use them.
Second, they host the highest amount of discardable communication activities (\textbf{Observation 6}).

